Adaptive Force-based Control for Legged Robots

Adaptive control can address model uncertainty in control systems. However, it is preliminarily designed for tracking control. Recent advancements in the control of quadruped robots show that force control can effectively realize agile and robust locomotion. In this paper, we present a novel adaptive force-based control framework for legged robots. We introduce a new architecture in our proposed approach to incorporate adaptive control into quadratic programming (QP) force control. Since our approach is based on force control, it also retains the advantages of the baseline framework, such as robustness to uneven terrain, controllable friction constraints, or soft impacts. Our method is successfully validated in both simulation and hardware experiments. While the baseline QP control has shown a significant degradation in the body tracking error with a small load, our proposed adaptive force-based control can enable the 12-kg Unitree A1 robot to walk on rough terrains while carrying a heavy load of up to 6 kg (50% of the robot weight). When standing with four legs, our proposed adaptive control can even allow the robot to carry up to 11 kg of load (92% of the robot weight) with less than 5-cm tracking error in the robot height.

==> Utils/TestCommands.tex <==
% File used to test the custom commands for various equations and variables used in the paper.

% Titles the section 
\section{Test Commands}

State Variable Definitions\\
$\roll \pitch \yaw \dRoll \dPitch \dYaw \omegaX \omegaY \omegaZ\\
\quatVector \posVector \angVelVector \velVector \rpyVector \rpyDotVector\\
\stateVector \stateVectorRed \inputVector\\
\rpyVector = \quatToRPY\\
\rpyDotVector = \omegaToRPYDot\angVelVector$\\\\

Simplified Dynamics\\
$\inputForceTorqueFunction = \inputForceTorque = \forceTorqueTransform\uToForceTorqueMat\BMat{\forceEstimate_1 \\ \vdots \\ \forceEstimate_s}\\
\simpleDynamics$\\\\

Direct Collocation Decision Variables\\
$\decisionArrayVector\\
\decisionArrayVectorFull$\\\\

Model Predictive Control Formulation\\
$\basicCostFunction\\
\basicCost = \MPCCostFull\\
\stateError = \stateErrorFull\\
\inputError = \inputErrorFull\\
\basicCostFunction = \MPCCostFunction$\\

% MPC Formulation (descriptive titles)
\begin{equation*}
	\begin{matrix}
		&\MPCMin
		&   & \MPCSum\pMat{\MPCCost}_{n,k} \\\\
		& \text{subject to}
		&	& \text{Dynamics} \\
		  &   &   & \dynamicsConstraint                \\\\
		  &   &   & \text{Foot placed on ground}       \\
		  &   &   & \groundConstraint                  \\\\
		  &   &   & \text{Kinematic leg limits}        \\
		  &   &   & \kinematicLegConstraint            \\\\
		  &   &   & \text{Foot stationary in stance}   \\
		  &   &   & \slipConstraint                    \\\\
		  &   &   & \text{Lateral force friction cone} \\
		  &   &   & \frictionConstraint{x}             \\
		  &   &   & \frictionConstraint{y}             
	\end{matrix}
\end{equation*}

% MPC Formulation (just equations)
\begin{equation*}
	\begin{matrix}
		&\MPCMin
		&   & \MPCSum\pMat{\MPCCost}_{n,k} \\\\
		& \text{subject to}
		&   & \dynamicsConstraint     \\
		  &   &   & \groundConstraint       \\
		  &   &   & \kinematicLegConstraint \\
		  &   &   & \slipConstraint         \\
		  &   &   & \frictionConstraint{x}  \\
		  &   &   & \frictionConstraint{y}  \\
	\end{matrix}
\end{equation*}

==> sections/hardware.tex <==
\section{\update{Robot Specification}}
\label{sec:RobotModel}
In this paper, we will validate our controller in the model of LASER (Legged-Agile-Smart-Efficient-Robot) mini. The LASER mini robot is a highly dynamic quadruped platform built from Unitree A1 robot (see \figref{fig:RobotDiagram}). The LASER mini has low-inertial legs and high torque density electric motors with planetary gear reduction, and it is capable of ground force control without using any force or torque sensors. The LASER mini robot uses these high-performance  actuators for all the hip, thigh, and knee joints to enable full 3D control of ground reaction forces. It is also equipped with contact sensors on each foot. 
\begin{figure}[bt!]
	\center
	\includegraphics[width=1.0\linewidth]{fig/hardware_config.jpg}
	\caption{{\bfseries Robot Configuration.}  Overview of LASER mini robot and leg configuration}
	\label{fig:RobotDiagram}
	
\end{figure}
%The LASER legs feature a large range of motion as presented in Figure \ref{fig:RobotDiagram}. The hip joints have a range of motion of $\pm$46${}^{\circ}$, the thigh joints have a range of motion from ${-60}^{\circ}$ to ${240}^{\circ}$ and the knee joints have a range from ${-154.5}^{\circ}$ to ${-52.5}^{\circ}$. The hip and knee designs allow the robot to operate identically forward, backward and flipped upside-down. 

		
Each of LASER mini's actuators consists of a custom high torque density electric motor coupled to a single-stage 9:1 planetary gear reduction. It can generate maximum joint torque of 33.5 ${Nm}$ and maximum joint speed of 21${Rad}/{s}$. The lower link is driven by a bar linkage which passes through the upper link. The legs are serially actuated, but to keep leg inertia low, the hip and knee actuators are co-axially located at the hip of each leg.

\vspace{-2.5em}
%The actuation capabilities of the LASER robot are summarized in Table \ref{tab:motor}.
% 	\begin{table}[bt!]
% 	%		\hspace{0.2cm}
% 	\centering
% 	\caption{Actuator Parameters}
% 	\begin{tabular}{cccc}
% 		\hline
% 		Parameter & Value & Units\\
% 		\hline
% 		Gear Ratio &   9   &   \\[.5ex]
% 		Max Torque   &  33.5 & ${Nm}$  \\[.5ex]
% 		Max Joint Speed    & 21  & ${Rad}/{s}$  \\[.5ex]
% 		\hline 
% 		\label{tab:motor}
% 	\end{tabular}
% \end{table}
